Diffusion Lens: Interpreting Text Encoders in Text-to-Image Pipelines

Text-to-image diffusion models (T2I) use a latent representation of a text prompt to guide the image generation process. However, the process by which the encoder produces the text representation is unknown. We propose the Diffusion Lens, a method for analyzing the text encoder of T2I models by generating images from its intermediate representations. Using the Diffusion Lens, we perform an extensive analysis of two recent T2I models. Exploring compound prompts, we find that complex scenes describing multiple objects are composed progressively and more slowly compared to simple scenes; Exploring knowledge retrieval, we find that representation of uncommon concepts requires further computation compared to common concepts, and that knowledge retrieval is gradual across layers. Overall, our findings provide valuable insights into the text encoder component in T2I pipelines.

==> 1.intro-old.tex <==
\section{Introduction}
\label{sec:intro}



While text-to-image (TTI) models have achieved great results in generating realistic images from natural text \cite{saharia2022photorealistic, rombach2022high}, the inner workings of these models remain largely unknown. 
In this paper we focus on the text encoder and explore the evolution of the prompt's representation throughout its layers. We focus on the representation of different concepts in the prompt and the relations between them that allows the model to later generate the corresponding image.  

Namely, we aim to analyze how the representation of a prompt progresses through the different layers of the text encoder.




We propose \method, a novel yet simple method to visualize the representation at each layer by generating images conditioned on these intermediate representations of the text encoder. 

We show that coherent images can be generated from almost all intermediate representations and that these representations capture different levels of abstraction and granularity.
Using \method, we are able to explore the relationship between different components prompts, including the obscurity or commonality of the concepts in the prompt, attributes such as the order and color of the components, and --- .  
Furthermore, we analyze the properties of the language model and discover interesting patterns and phenomena in its encoding process.

Using \method, we conclude that \da{for complex prompts, containing multiple concepts, ?} at the early layers of the text encoder, representations are characterized as "bags of concepts", i.e., no relations have yet been established. In contrast, images produced from the later layers provide a more accurate representation of the sentence's relations. Furthermore, we find that common concepts appear already in images generated from early layers, while uncommon concepts only appear in the later layers. See Figure \ref{fig:aye-aye}, \ref{fig:dog}. 

Our contribution is two-fold:
\begin{itemize}
    \item 
    We demonstrate for the first time that intermediate representations can be used as conditions for diffusion. %
    \item 
    Our method is demonstrated in various cases, providing previously unknown insights into the flow of information in transformer encoders. 
\end{itemize}

We believe that this method can be used to examine more phenomena in TTI models. 





==> 4.experiments_old.tex <==


\section{Experimental Setup}
\label{sec:experimental_setup}

In the following sections, we use \method to perform visuolinguistic analyses of the text encoder in text-to-image models.

\paragraph{Models.}
The experiments are performed on Stable Diffusion 2.1 (denoted \emph{SD}) \cite{stable_diffusion} and Deep Floyd (denoted \emph{DF}) \cite{deep_floyed}. 
SD is an open-source implementation of latent diffusion \cite{rombach2022high}, with OpenCLIP-ViT/H \cite{ilharco_gabriel_2021_5143773} as the text-encoder.
DF is another open-source implementation of latent diffusion inspired by \cite{saharia2022photorealistic}, with frozen T5-XXL as the text encoder \cite{raffel2020exploring}.

\paragraph{Data.}
We curate lists of prompts for each analysis, which we describe separately for each experiment. Each prompt is used to generate images that are conditioned on different layers in the model, and we use different seeds to generate each image.

\paragraph{Evaluation.} For every experiment we ask questions regarding the images in every layer, e.g., ``Does the prompt correspond to the generated image''; or, when there are two objects in the prompt, ``Does object A appear in the generated image?''. We describe the questions in detail for every experiment below. For each experiment, we used a small set to perform human annotations (by the authors of the paper) as well as GPT-4 \cite{openai2023gpt4} annotations. We then measured the agreement between the human annotations and GPT-4, and if it is satisfying, we perform a larger-scale experiment with GPT-4 annotations only. Otherwise, we increase the scale and continue with manual annotations. \ho{This needs editing after we finish with annotations. Also, explain why other automatic annotation methods such as CLIP or BLIP would not work well. Maybe disucuss "gpt-judge" related work.} \yb{yeah, need more info on the annotation process, as well as human agreement results, and when gpt4 works well or not}


 





\section{Conceptual Combination}

Conceptual combination is the cognitive process by which at least two existing basic concepts are combined to generate a new higher-order, composite concept \cite{WU2009173}.
Conceptual combination is at the core of knowledge representation, since it asks how a complex noun phrase's meaning connects to its component parts \cite{hampton2013conceptual}.
Text-to-image diffusion models are popular for their ability to generalize beyond their training data, creating composite concepts \cite{ramesh2022hierarchical}.
This section utilizes \method~to visualize the process by which the text encoder creates the composite concept.

\paragraph{Colors and conjuction.} We compile three lists of prompts:
(1) a list of objects (e.g., ``a dog''); (2) a list of objects with color description (e.g., ``a red dog''); and (3) a list where each prompt describes two objects with color description(e.g., ``a red dog and a white cat'').
For each layer that we produce an image for, we ask whether the prompt correctly describes the generated image.
Since we are interested in analyzing a full representation building, we only keep prompts that the diffusion model was able to generate correctly \ho{need better wording here...}.
Furthermore, we investigate how the conceptual combination is emerging throughout the layers.
For each layer we ask the following six questions: (a) does object A appear in the image? (b) does object B appear in the prompt? (c) does color A appear in the image? (d) does color B appear in the image? (e) does object A appear in the image in the right color? (f) does object B appear in the right color?

\paragraph{Results.} Figure [TODO] plots the results for each of the prompt list, across layers. As the concept described in the prompt is simpler, it already emerges in earlier layers. For the prompts that describe single concepts, the image emerges already around layers X, Y, while for the prompts with color descriptors that happens only around layers Z, W and for the preposition prompts it happens around layers A, B.

\paragraph{Prepositions.} We use two lists of prompts: (1) a list of objects, same as in the first experiment; and (2) a list where each prompt describes two object and a preposition, for example, ``A cat under a chair''.
For each layer, we again ask whether the prompt correctly describes the image.
Furthermore, we ask three questions: (a) does object A appear in the sentence? (b) does object B appear in the sentence? (c) does the preposition appear in the sentence?

\paragraph{Results.} \ho{todo... probably will be similar results to the first experiment. consider combining once written.}



\paragraph{Head and dependent order of generation.} TODO

\paragraph{Compounds.} TODO

\section{Knowledge Encoding}
 
\paragraph{Common and Rare Concepts}

\paragraph{Gradual Retrieval of Knowledge.}

\paragraph{Gradual refinement of features.}

\section{Additional Qualitative Results}




\begin{figure}[!htb]
\centering
\includegraphics[width=\linewidth]{assets/plots/Human_Annotations_-_common_animals_-_DF.png}
\caption{Average scores of the human annotations over common animals. Early layers represent well the animals.}\label{fig:common_animals}
\end{figure}


\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]
{assets/plots/Visual_animals_3.png}
\caption{Human annotation average over the presence of an animal, mammal, and specific features of common (dashed line) and uncommon (full line) animals. While common animals display correct features in the early layers, uncommon animals take more time to achieve animal or mammal representation, and their specific characteristics are revealed only in the later layers.}
\label{fig:common_vs_uncommon_animals}
\end{figure}



 



\begin{figure}[!h]
\centering
\includegraphics[width=\linewidth]{assets/plots/Human_Annotations_-_color_-_DF.png}
\caption{Human annotation average over the presence of either of the objects, and both objects with the correct colors.}
\label{fig:two_things_color}
\end{figure}



==> additional_results.tex <==
\section{Additional Results}
\ho{TODO decide how this should be merged into the paper}
\paragraph{Mix of concepts}
\citet{rassin2022dalle}, depicted concepts that can be interpreted in more than one way, such as a bat, which can be viewed as both an animal and a tool, and often ends up in images that contain both. Here we see a similar pattern in the early layers. Earlier layers tend to have

\paragraph{First layers}
The 7 first layers in Deep Floyd look very different from the later layers, although many times, the patterns correspond to the prompt that exists in the images, especially colors. We believe that our method fails to generate coherent images from these layers due to a big gap in the distribution of the weights in their layers. Future work might look into this phenomenon and try to find a method that would work on these layers. 
In Stable Diffusion 2.1 we see a similar pattern, although these images are less colorful. The five first layers have different textures. The images in later layers look more similar to regular images.


==> main_plot.tex <==









==> previour_comments.tex <==

































































